Spatial-Language Attention Policies for Efficient Robot Learning

Despite great strides in language-guided manipulation, existing work has been constrained to table-top settings. Table-tops allow for perfect and consistent camera angles, properties are that do not hold in mobile manipulation. Task plans that involve moving around the environment must be robust to egocentric views and changes in the plane and angle of grasp. A further challenge is ensuring this is all true while still being able to learn skills efficiently from limited data. We propose Spatial-Language Attention Policies (SLAP) as a solution. SLAP uses three-dimensional tokens as the input representation to train a single multi-task, language-conditioned action prediction policy. Our method shows an 80% success rate in the real world across eight tasks with a single model, and a 47.5% success rate when unseen clutter and unseen object configurations are introduced, even with only a handful of examples per task. This represents an improvement of 30% over prior work (20% given unseen distractors and configurations). We see a 4x improvement over baseline in mobile manipulation setting. In addition, we show how SLAPs robustness allows us to execute Task Plans from open-vocabulary instructions using a large language model for multi-step mobile manipulation. For videos, see the website: https://robotslap.github.io

==> 06discussion.tex <==
\label{sec:Discussion}



Our experiments show that \slap{} has a number of advantages over previous work.
We also observe that \slap{} predicted consistently successful actions for opening the top and bottom drawers. While the top drawer handle is a small leather loop, the bottom drawer handle is a slender cylindrical rod. PerAct produces more inaccurate predictions for the small loop on the drawer, while failing completely to grasp the bottom handle. See Fig.~\ref{fig:peract-v-slap} for an example. We note that our $\pi_I$ has a finer granularity than PerAct's representation.
%This indicates that \slap{} encodings might have a better understanding of local and fine structures due to its high-dimensional input-space.

% \cpax{I really don't agree with this paragraph:
% Since the expert demonstrator also implicitly follows rules about collision-avoidance and task semantics, those are captured by $\pi_R$ as well.
% In contrast, PerAct learns each keyframe with respect to the entire scene rather than a local context, this results in predicted actions not describing a smooth trajectory or predicting infeasible actions in the worst case (see Fig.~\ref{fig:peract-discontinuities}). Such results highlight PerAct's reliance on a collision-aware motion planner by design, while \slap{} does not have such a limitation. Along similar lines, we notice more motion planning failures during PerAct rollouts specifically due to orientation predictions.
% }

%\slap{} suffers from a different problem due to its architecture design. We find repeated confusion between the white basket and the white drawer for the placing skill. This could be due to our emphasis on local structure; it is hard to distinguish between planar drawer insides and planar basket insides. It could also be due to the similar color, which is something which should be addressed with more data, better augmentation, or by using pretrained image features. 

\textbf{Locality Loss.} We observed reduced object confusion with locality loss when comparing to a version of \slap{} trained without it. Before adding the locality loss, the attention for a skill would be spread farther around the scene -- spreading to the bottom drawer from top and vice-versa for example. This led to confusion and lower success rates on drawer-related tasks (previously, 0\% on bottom drawer and 70\% on top drawer from a 9-task model trained with data augmentation). 
% \cpax{Priyam - add a number from the previous version of the paper here?}. 
However, the locality loss encouraged attention to be concentrated tightly on the relevant surfaces of the implicated object, as seen in Fig.~\ref{fig:locality-loss-tight-attention-mask}.
% We observed this led to less confusion with object placed near implicated object during in-domain testing. In other words, this loss helped significantly with in-domain robustness.

\begin{figure}[b]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/results_discussion/peract_vs_slap.pdf}
    \caption{Output for interaction action predicted by PerAct (left) and interaction point predicted by \slap{} (right) for the same input. We see a trend where $\pi_I$ predictions for finer details are consistently more optimal} 
    \label{fig:peract-v-slap}
\end{figure}

\begin{figure}[bt]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/results_discussion/locality_loss.pdf}
    \caption{A comparison of attention masks with (right) and without (left) the locality loss. Attention is more focused on relevant structures and less spread to irrelevant structures in the right image. The top row shows the attention mask for opening the top drawer: the previous model (left) spreads attention to the bottom handle due to its association with the "open" skill, while the new model (right) focuses only on the top drawer. Attention is more concentrated on handle for the "open bottom drawer" skill in the bottom row.}
    \label{fig:locality-loss-tight-attention-mask}
\end{figure}



==> a1notes.tex <==
\section{Intro notes}
Goal: take in point clouds and use them to predict short trajectory segments that we can use for carrying out multi-step policies.

% We will use a LLM to make predictions for what the next action or 2 should be.

% \begin{itemize}
%     \item 3 - collect more data + langauge annotations
%     \item 4 - training larger and larger models 
%     \item 5 - more robot experiments on complex tasks
% \end{itemize}

% download OPT, do some completion queries on our learned set of models + show multi step task execution (lazy say can)

% Chris - get it running on a second robot (the stretch)
Tasks:
\begin{itemize}
    \item open close top drawer
    \item open close bottom drawer
    \item open close microwave
    \item pickup x (color and category based task)
\end{itemize}

\begin{itemize}
    \item place x in drawer micro etc
\end{itemize}


\subsection{Plans}

\textbf{Benchmarking.} We want to:
\begin{itemize}
    \item Run --10-- 8 tasks on real robot (RoboPen), with 1 task chain example
    \item Compare against PtNet++ based regressor (ours w/out the classification head)
    \item Compare against our V0 (PT-model)
\end{itemize}


\section{Experiment Notes}

\subsection{Ablations}

compare to:
\begin{itemize}
    \item no regularization loss
    \item no masking
    \item no language? language only?
    \item direct point-cloud to object prediction
    \item no augmentation - remove those
\end{itemize}

\textbf{On dropout.} We tried using dropout (rate of $25\%$) to see if this would cause any difficulties or help get the masks to converge more quickly on relevant parts of the image. I think it ends up being just fine, but it's definitely not the best; it doesn't seem to matter very much.

\textbf{On training.} With a handful of ``reach target'' examples with different targets, validation loss really seems to lag behind train for a while. Eventually (maybe after 2000-5000 steps for 12 examples) it falls off a cliff and the two start to be much more aligned. This might be related to learning rate.

\textbf{On mask values.} Mask values should be pretty high for the best entries and pretty low (close to zero) for others. Things that encourage this: adding a mask regularization term. \textbf{\textit{without this term, we would expect worse generalization and worse test-time performance, especially with respect to distractors.}}


\subsection{Comparisons}

\begin{itemize}
    \item r3m, clip, and imagenet weights - we will use ViT or resnet weights and behavioral cloning
    \item direct prediction of the goal?
    \item pointnet++ policy as per in Shohin's paper?
\end{itemize}

More notes:
\begin{itemize}
    \item PointConv embeddings which classify closest centroid and use the same embeddings to train ori/pos of next keyframe
    \item Trained segmentation network whose feature layer can be used for both closest point prediction classification + ori/pos prediction
    \item Pure transformer Seq2Seq training where each word and each centroid is a word, given the classified closest centroid: together they predict the next keypoint
\end{itemize}


\subsection{Ongoing results}

\textbf{11/04 - Classification model with feature propagation}.\\
The classification model does pretty well as far as structure is concerned however it seems like language gets diffused to not send enough signals. Look at the attached results below\ref{fig:11-04}.
\begin{figure*}
\includegraphics[width=0.49\textwidth]{figs/placeholder/error-mode-lang-2-blue-true.png}
\includegraphics[width=0.49\textwidth]{figs/placeholder/error-mode-language-marron-true.png}
\caption{11/04 - Example of failure modes. While structurally our model learns which structures or shapes in the environment make sense, however not able to distinguish between colors which are primarily communication through rgb and language features. Left is supposed to tag a ``blue ball'' while the right one is supposed to tag the ``maroon'' ball}
\label{fig:11-04}
\end{figure*}

\textbf{11/06 - Bug in previous model}\\
While updating classification model realized old voxel-only classification model(which was also doing well after 40-50 epochs) had a bug where \texttt{forward} was returning features before they were updated by perceiverIO. Trying out experiment with voxel-only classification with that bug fixed so regression can get more information [\href{https://github.com/cpaxton/home_robot/commit/a4a8d8cbade90dac3bd8fe183ec5bd93aceafc6f}{Commit-link}, \href{https://wandb.ai/larping/larp-pt_query-query_pointnet_voxel_classifier?workspace=user-priparashar}{WANDB Project Link}]

After 25 epochs (1100 seconds), model still confuses between blue and green color. I remember this behavior from 1st time we tried this model. After training for another 1100 seconds, converges around 45-50 epochs. Still confuses blue with red, got 14/15 validation tasks.

\textit{Morning.} Regression with just an MLP added to regression features overfits and does REALLY well on valid when closest\_pt supervision is perfect. Checked using dataloader grnd truth as input. However, it blows up when classifier model is used during validation. Did an experiment and found that classifier-loss in trying to find the closest pt is in 10s of cm range, going up to 50-60cm. Obviously it doesn't work.

\textit{Afternoon.}
\texttt{pt\_query.\_query\_radius} is a sensitive parameter, 0.05 does \href{https://wandb.ai/larping/larp-pt_query-query_pointnet_voxel_classifier?workspace=user-priparashar}{spectacularly bad}. pt\_enc also seems to make the model worse. Trying out with and without pt\_enc without my LR schedule. 

\textbf{11/06 - Planning}

\begin{itemize}
    \item Real robot-results - single-step tasks
    \item Update RLBench so object distribution is larger than peract bbox
    \item Train PerAct and C2F-ARM on all relevant tasks with larger bbox
    \item Run PerAct and C2F-ARM on robot data with larger bbox
    \item Scale up tasks
\end{itemize}

\textbf{11/10}
\textit{Status}
Have RoboPen data for picking up the box (10 training, 3 validation). Overfitting yesterday on 1 tiger toy reach example seemed to work. Depth data did not look great so did not try for multi-step pear pick-up. It was very hard to understand keyframe relabeling. 
\textit{Plan}
\begin{itemize}
    \item Confirm relabeling makes sense (1st keyframe is ``look at'' pose, with relevant-point being 3rd keyframe which is the interaction keyframe; for every keyframe the input is 1st frame of its segment with interaction point being labeled as the relevant point to be classified)
    \item Train classifier on this data
    \item Train regression on this data
    \item Tune regression weights on this data
\end{itemize}

\subsection{Ideas to try}

\begin{itemize}
    \item \textbf{Classification} Multi-label loss, where all points within 5mm of the closest points are candidates for true label. Use \href{https://pytorch.org/docs/stable/generated/torch.nn.NLLLoss.html}{NLLLoss} through this \href{https://discuss.pytorch.org/t/categorical-cross-entropy-loss-function-equivalent-in-pytorch/85165/4}{example}
\end{itemize}
